Quasi-local black hole horizons

This article introduces the subject of quasi-local horizons at a level suitable for physics graduate students who have taken a first course on general relativity. It reviews properties of trapped surfaces and trapped regions in some simple examples, general properties of trapped surfaces including their stability properties, the definitions and some applications of dynamical-, trapping-, and isolated-horizons.

==> figs/inkheader.tex <==
\usepackage{mathrsfs}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amssymb}
